Integrating Locality-Aware Attention with Transformers for General Geometry PDEs

Neural operators have emerged as promising frameworks for learning mappings governed by partial differential equations (PDEs), serving as data-driven alternatives to traditional numerical methods. While methods such as the Fourier neural operator (FNO) have demonstrated notable performance, their reliance on uniform grids restricts their applicability to complex geometries and irregular meshes. Recently, Transformer-based neural operators with linear attention mechanisms have shown potential in overcoming these limitations for large-scale PDE simulations. However, these approaches predominantly emphasize global feature aggregation, often overlooking fine-scale dynamics and localized PDE behaviors essential for accurate solutions. To address these challenges, we propose the Locality-Aware Attention Transformer (LA2Former), which leverages K-nearest neighbors for dynamic patchifying and integrates global-local attention for enhanced PDE modeling. By combining linear attention for efficient global context encoding with pairwise attention for capturing intricate local interactions, LA2Former achieves an optimal balance between computational efficiency and predictive accuracy. Extensive evaluations across six benchmark datasets demonstrate that LA2Former improves predictive accuracy by over 50% relative to existing linear attention methods, while also outperforming full pairwise attention under optimal conditions. This work underscores the critical importance of localized feature learning in advancing Transformer-based neural operators for solving PDEs on complex and irregular domains.

==> figures/KNN_header.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{figures/sources/KNN_param.png}
\end{center}
\caption{\l2 relative error varies w.r.t. the number of layers (Left) and width (right) of ONO on Pipe and Elasticity benchmarks}
\label{fig:case_study}
\end{figure}

==> figures/PDE_sample.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/sources/PDE_sample.jpeg}
\end{center}
\vspace{-0.5cm}
\caption{Examples of PDE-governed tasks, including solid (left) and fluid (right) physics, whose solving processes are approximating complex input-output mappings in discretized high-dimensional coordinate spaces. All the tasks are covered in our experiments.}
% \vspace{-0.2cm}
\label{fig:benchmark1}
\end{figure*}

==> figures/scale_knn.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.98\columnwidth]{figures/sources/scale_knn.png} % Updated image path and size
\end{center}
\vspace{-0.5cm}
\caption{Effect of local attention window size. Relative \( L_2 \) error (solid lines) and runtime per epoch (dashed lines) are plotted against \( K \) values for Darcy and Elasticity datasets.} 
% \vspace{-0.2cm}
\label{fig:scale_knn}
\end{figure}

==> tables/runtime.tex <==
\begin{table}[t]
\caption{Runtime comparison for different models. All models use a batch size of 1 on the elasticity (972 mesh points) dataset. The hidden state of the single-head attention mechanism is configured with 128 dimensions.} 
\centering  % 표 중앙 정렬

\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Model} & \textbf{FNO} & \textbf{Galerkin} & \textbf{LSM} & \textbf{LA2Former}\\
    \midrule
    Runtime (s) & 3.81 & 9.88 & 9.05 & 12.15   \\
    \bottomrule
\end{tabular}
\label{tab:Runtime}
}
\vspace{-0.2cm}
\end{table}


==> tables/table3.tex <==
\begin{table}[h]
\caption{Ablation study on the number of K.}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\textbf{\#Memory}} & \multicolumn{1}{c|}{\textbf{\#Time}} & \multicolumn{2}{c|}{\textbf{Relative L2}} \\
    \hline
    \multicolumn{2}{|c|}{\textbf{Ablations}} & (GB) & (s/epoch) & \textbf{Elasticity} & \textbf{Darcy} \\
    \hline
    \multirow{10}{*}{\centering \textbf{\#. of $K$}}
        & 9     & 0.60 & 37.76 & 0.0148 & 0.0386 \\
        & 16     & 0.60 & 37.82 & 0.0071 & 0.0096 \\
        & 25    & 0.61 & 37.96 & 0.0067 & 0.0067 \\
        & 36    & 0.62 & 38.00 & 0.0067 & 0.0063 \\
        & 49    & 0.64 & 38.18 & 0.0064 & 0.0059 \\
        & 64    & 0.68 & 38.31 & 0.0061 & 0.0055 \\
    \hline
    \multicolumn{2}{|c|}{\textbf{Regular Squares}} & / & / & / & 0.0088 \\
    \hline
\end{tabular}
\label{tab:ablation}
}
\end{table}


